The nuclear gas disk of NGC 1566 dissected by SINFONI and ALMA

We present the results of near-infrared H- and K-band European Southern Observatory SINFONI integral field spectroscopy of the Seyfert galaxy NGC 1566. We investigate the central kpc of this nearby galaxy, concentrating on excitation conditions, morphology, and stellar content. NGC 1566 was selected from our NUGA (-south) sample and is a ringed, spiral galaxy with a stellar bar. We present emission and absorption line measurements in the central kpc of NGC 1566. Broad and narrow Br{\gamma} lines were detected. The detection of a broad Br{\gamma} component is a clear sign of a super-massive black hole in the center. Blackbody emission temperatures of ~1000 K are indicative of a hot dust component, the torus, in the nuclear region. The molecular hydrogen lines, hydrogen recombination lines, and [FeII] indicate that the excitation at the center is coming from an AGN. The central region is predominantly inhabited by molecular gas, dust, and an old K-M type giant stellar population. The molecular gas and stellar velocity maps both show a rotation pattern. The molecular gas velocity field shows a perturbation toward the center that is typical for bars or spiral density waves. The molecular gas species of warm H_2(1-0)S(1) and cold ^{12}CO(3-2) gas trace a nuclear gas disk of about 3" in radius with a nuclear spiral reaching toward the nucleus. From the equivalent width of H_2(1-0)S(1) a molecular ring with r<~3" can be inferred. This spiral seems to be an instrument that allows gas to fall toward the nucleus down to <50 pc scales. The excitation of molecular hydrogen in the nuclear gas disk is not clear but diagnostic diagrams show a distinction between the nuclear region and a <9 Myr old star forming region at the southwestern spiral arm. Possibly shocked gas is detected ~2" from the center, which is visible in dispersion maps of H$_2$(1-0)S(1) and ^{12}CO(3-2) and in the 0.87 mm continuum.

==> regionEW.tex <==
\begin{table*}[htbp]
\centering
\caption{Equivalent width}
\begin{tabular}{c c c c c c c}
\hline\hline
%\multicolumn{7}{c}{Equivalent width} \\
  & Center $r=1\arcsec$ & Center $r=5\arcsec$ & Center $r=$~PSF & SFr & SF PSF & cPSF \\
\hline
 \ion{Si}{i} & $2.64$ & $2.34$ & $2.60$ & $2.38$ & $2.31$ & $2.47$ \\
%% $\lambda$ 1.589 \mic \\
 CO(6-3) & $6.45$ & $6.52$ & $6.24$ & $6.71$ & $7.05$ & $5.88$ \\
%% $\lambda$ 1.619 \mic \\
% $[$\ion{Fe}{ii}$]$ & $5.93\pm0.68$ & $...$ & $4.82\pm0.38$ & $0.21\pm0.09$ & $0.06\pm0.02$ & $2.39\pm0.13$ \\
%% $\lambda$ 1.644 \mic \\
% H$_2$(1-0)S(3) & $3.80\pm0.33$ & $15.15\pm3.18$ & $2.35\pm0.19$ & $0.57\pm0.05$ & $0.14\pm0.01$ & $0.93\pm0.07$ \\
%% $\lambda$ 1.957 \mic \\
% H$_2$(1-0)S(2) & $1.66\pm0.18$ & $5.46\pm1.35$ & $1.01\pm0.10$ & $0.28\pm0.03$ & $0.08\pm0.01$ & $0.39\pm0.04$ \\
%% $\lambda$ 2.033 \mic \\
% \ion{He}{i} & $0.51\pm0.14$ & $...$ & $0.42\pm0.09$ & $0.17\pm0.02$ & $0.05\pm0.006$ & $0.23\pm0.04$ \\
%% $\lambda$ 2.058 \mic \\
% H$_2$(1-0)S(1) & $3.41\pm0.15$ & $11.21\pm1.2$ & $2.25\pm0.09$ & $0.52\pm0.03$ & $0.13\pm0.008$ & $0.96\pm0.03$ \\
%% $\lambda$ 2.122 \mic \\
 Br$\gamma$ & $0.55$ & $...$ & $0.79$ & $1.60$ & $2.59$ & $1.03$ \\
%% $\lambda$ 2.166 \mic \\
% H$_2$(1-0)S(0) & $1.04\pm0.12$ & $3.68\pm1.06$ & $0.64\pm0.07$ & $0.17\pm0.02$ & $0.05\pm0.005$ & $0.25\pm0.03$ \\
%% $\lambda$ 2.223 \mic \\
% H$_2$(2-1)S(1) & $0.55\pm0.11$ & $...$ & $0.35\pm0.07$ & $0.11\pm0.02$ & $0.03\pm0.005$ & $0.14\pm0.03$ \\
%% $\lambda$ 2.247 \mic \\
% H$_2$(1-0)Q(1) & $3.68\pm0.35$ & $33.64\pm8.44$ & $2.23\pm0.17$ & $0.74\pm0.11$ & $0.16\pm0.02$ & $0.86\pm0.07$ \\
%% $\lambda$ 2.408 \mic \\
%% H$_2$(1-0)Q(2) & $0.79\pm...$ & $290\pm...$ & $...$ & $...$ & $0.06\pm...$ & $115\pm...$ \\
%% 2.414 \\
% H$_2$(1-0)Q(3) & $3.23\pm0.24$ & $49.70\pm5.7$ & $1.80\pm0.12$ & $0.81\pm0.11$ & $0.17\pm0.03$ & $0.69\pm0.05$ \\
%% $\lambda$ 2.422 \mic \\
 \ion{Na}{i} & $3.41$ & $3.27$ & $3.26$ & $3.61$ & $3.50$ & $3.22$ \\
% $\lambda$ 2.208 \mic \\
 \ion{Ca}{i} & $4.51$ & $4.26$ & $4.53$ & $4.79$ & $4.73$ & $4.70$ \\
% $\lambda$ 2.263 \mic \\
 CO(2-0) & $15.84$ & $16.91$ & $14.68$ & $18.45$ & $18.07$ & $13.50$ \\
% $\lambda$ 2.294 \mic \\
\hline

%\multicolumn{3}{l}{\tiny Note: The line flux and FWHM were measured with a ten pixel radius circular aperture (only full pixel were taken into account) centered so that all of the measured emission lines contribute in an adequate ratio. The FWHM is not corrected for instrumental broadening, which is about 225$kms^{-1}$ in H-band and 140$kms^{-1}$ in K-band.}
%\footnotetext[1]{Intergrated over a ten pixel radius aperture.}
\end{tabular}
\tablefoot{
Equivalent width of the stellar absorption features and of \brg\ given in $\AA$ of all discussed regions (see also Fig.~\ref{fig:lines1} for abbreviations). For all absorption features the line range and continuum range were taken from \citet{mannucci_near-infrared_2001} and the hot dust component in the center was subtracted prior to measuring the EW.
}
\label{tab:regionEW}
\end{table*}


==> regionEW2.tex <==
\begin{table}[htbp]
\centering
\caption{Equivalent width 2}
%\begin{tabular}{c c c c c c c}
%\hline\hline
%%\multicolumn{7}{c}{Equivalent width} \\
%  & Center $r=1\arcsec$ & Center $r=5\arcsec$ & Center $r=$~PSF & SFr & SF PSF & cPSF \\
%\hline
% \ion{Si}{i} & $2.28$ & $2.55$ & $2.15$ & $2.51$ & $2.33$ & $1.90$ \\
%%% $\lambda$ 1.589 \mic \\
% CO(6-3) & $3.43$ & $3.68$ & $3.37$ & $3.81$ & $3.66$ & $3.24$ \\
%%% $\lambda$ 1.619 \mic \\
%% $[$\ion{Fe}{ii}$]$ & $5.93\pm0.68$ & $...$ & $4.82\pm0.38$ & $0.21\pm0.09$ & $0.06\pm0.02$ & $2.39\pm0.13$ \\
%%% $\lambda$ 1.644 \mic \\
%% H$_2$(1-0)S(3) & $3.80\pm0.33$ & $15.15\pm3.18$ & $2.35\pm0.19$ & $0.57\pm0.05$ & $0.14\pm0.01$ & $0.93\pm0.07$ \\
%%% $\lambda$ 1.957 \mic \\
%% H$_2$(1-0)S(2) & $1.66\pm0.18$ & $5.46\pm1.35$ & $1.01\pm0.10$ & $0.28\pm0.03$ & $0.08\pm0.01$ & $0.39\pm0.04$ \\
%%% $\lambda$ 2.033 \mic \\
%% \ion{He}{i} & $0.51\pm0.14$ & $...$ & $0.42\pm0.09$ & $0.17\pm0.02$ & $0.05\pm0.006$ & $0.23\pm0.04$ \\
%%% $\lambda$ 2.058 \mic \\
%% H$_2$(1-0)S(1) & $3.41\pm0.15$ & $11.21\pm1.2$ & $2.25\pm0.09$ & $0.52\pm0.03$ & $0.13\pm0.008$ & $0.96\pm0.03$ \\
%%% $\lambda$ 2.122 \mic \\
% Br$\gamma$ & $0.55$ & $...$ & $0.79$ & $1.60$ & $2.59$ & $1.03$ \\
%%% $\lambda$ 2.166 \mic \\
%% H$_2$(1-0)S(0) & $1.04\pm0.12$ & $3.68\pm1.06$ & $0.64\pm0.07$ & $0.17\pm0.02$ & $0.05\pm0.005$ & $0.25\pm0.03$ \\
%%% $\lambda$ 2.223 \mic \\
%% H$_2$(2-1)S(1) & $0.55\pm0.11$ & $...$ & $0.35\pm0.07$ & $0.11\pm0.02$ & $0.03\pm0.005$ & $0.14\pm0.03$ \\
%%% $\lambda$ 2.247 \mic \\
%% H$_2$(1-0)Q(1) & $3.68\pm0.35$ & $33.64\pm8.44$ & $2.23\pm0.17$ & $0.74\pm0.11$ & $0.16\pm0.02$ & $0.86\pm0.07$ \\
%%% $\lambda$ 2.408 \mic \\
%%% H$_2$(1-0)Q(2) & $0.79\pm...$ & $290\pm...$ & $...$ & $...$ & $0.06\pm...$ & $115\pm...$ \\
%%% 2.414 \\
%% H$_2$(1-0)Q(3) & $3.23\pm0.24$ & $49.70\pm5.7$ & $1.80\pm0.12$ & $0.81\pm0.11$ & $0.17\pm0.03$ & $0.69\pm0.05$ \\
%%% $\lambda$ 2.422 \mic \\
% \ion{Na}{i} & $2.87$ & $2.59$ & $2.77$ & $2.93$ & $2.90$ & $2.76$ \\
%% $\lambda$ 2.208 \mic \\
% \ion{Ca}{i} & $2.29$ & $2.16$ & $2.22$ & $2.33$ & $2.31$ & $2.25$ \\
%% $\lambda$ 2.263 \mic \\
% CO(2-0) & $10.14$ & $10.28$ & $9.55$ & $10.94$ & $10.76$ & $9.10$ \\
%% $\lambda$ 2.294 \mic \\
%\hline

\begin{tabular}{c c c}
\hline\hline
%\multicolumn{7}{c}{Equivalent width} \\
  & SF PSF & cPSF \\
\hline
 \ion{Si}{i} & $2.33$ & $1.90$ \\
%% $\lambda$ 1.589 \mic \\
 CO(6-3) & $3.66$ & $3.24$ \\
%% $\lambda$ 1.619 \mic \\
% $[$\ion{Fe}{ii}$]$ & $5.93\pm0.68$ & $...$ & $4.82\pm0.38$ & $0.21\pm0.09$ & $0.06\pm0.02$ & $2.39\pm0.13$ \\
%% $\lambda$ 1.644 \mic \\
% H$_2$(1-0)S(3) & $3.80\pm0.33$ & $15.15\pm3.18$ & $2.35\pm0.19$ & $0.57\pm0.05$ & $0.14\pm0.01$ & $0.93\pm0.07$ \\
%% $\lambda$ 1.957 \mic \\
% H$_2$(1-0)S(2) & $1.66\pm0.18$ & $5.46\pm1.35$ & $1.01\pm0.10$ & $0.28\pm0.03$ & $0.08\pm0.01$ & $0.39\pm0.04$ \\
%% $\lambda$ 2.033 \mic \\
% \ion{He}{i} & $0.51\pm0.14$ & $...$ & $0.42\pm0.09$ & $0.17\pm0.02$ & $0.05\pm0.006$ & $0.23\pm0.04$ \\
%% $\lambda$ 2.058 \mic \\
% H$_2$(1-0)S(1) & $3.41\pm0.15$ & $11.21\pm1.2$ & $2.25\pm0.09$ & $0.52\pm0.03$ & $0.13\pm0.008$ & $0.96\pm0.03$ \\
%% $\lambda$ 2.122 \mic \\
% Br$\gamma$ & $2.59$ & $1.03$ \\
%% $\lambda$ 2.166 \mic \\
% H$_2$(1-0)S(0) & $1.04\pm0.12$ & $3.68\pm1.06$ & $0.64\pm0.07$ & $0.17\pm0.02$ & $0.05\pm0.005$ & $0.25\pm0.03$ \\
%% $\lambda$ 2.223 \mic \\
% H$_2$(2-1)S(1) & $0.55\pm0.11$ & $...$ & $0.35\pm0.07$ & $0.11\pm0.02$ & $0.03\pm0.005$ & $0.14\pm0.03$ \\
%% $\lambda$ 2.247 \mic \\
% H$_2$(1-0)Q(1) & $3.68\pm0.35$ & $33.64\pm8.44$ & $2.23\pm0.17$ & $0.74\pm0.11$ & $0.16\pm0.02$ & $0.86\pm0.07$ \\
%% $\lambda$ 2.408 \mic \\
%% H$_2$(1-0)Q(2) & $0.79\pm...$ & $290\pm...$ & $...$ & $...$ & $0.06\pm...$ & $115\pm...$ \\
%% 2.414 \\
% H$_2$(1-0)Q(3) & $3.23\pm0.24$ & $49.70\pm5.7$ & $1.80\pm0.12$ & $0.81\pm0.11$ & $0.17\pm0.03$ & $0.69\pm0.05$ \\
%% $\lambda$ 2.422 \mic \\
% \ion{Na}{i} & $2.76$ \\
% $\lambda$ 2.208 \mic \\
% \ion{Ca}{i} & $2.31$ & $2.25$ \\
% $\lambda$ 2.263 \mic \\
 CO(2-0) & $10.76$ & $9.10$ \\
% $\lambda$ 2.294 \mic \\
\hline

%\multicolumn{3}{l}{\tiny Note: The line flux and FWHM were measured with a ten pixel radius circular aperture (only full pixel were taken into account) centered so that all of the measured emission lines contribute in an adequate ratio. The FWHM is not corrected for instrumental broadening, which is about 225$kms^{-1}$ in H-band and 140$kms^{-1}$ in K-band.}
%\footnotetext[1]{Intergrated over a ten pixel radius aperture.}
\end{tabular}
\tablefoot{
Equivalent width of the stellar absorption features and of \brg\ given in $\AA$ of the discussed regions (see also Fig.~\ref{fig:lines1} for abbreviations). For all absorption features the line range and continuum range were taken from \citet{origlia_1.5-1.7_1993} and the hot dust component in the center was subtracted prior to measuring the EW.
}
\label{tab:regionEW2}
\end{table}

